Seeded graph matching for the correlated Gaussian Wigner model via the projected power method

In the \emph{graph matching} problem we observe two graphs $G,H$ and the goal is to find an assignment (or matching) between their vertices such that some measure of edge agreement is maximized. We assume in this work that the observed pair $G,H$ has been drawn from the Correlated Gaussian Wigner (CGW) model -- a popular model for correlated weighted graphs -- where the entries of the adjacency matrices of $G$ and $H$ are independent Gaussians and each edge of $G$ is correlated with one edge of $H$ (determined by the unknown matching) with the edge correlation described by a parameter $\sigma\in [0,1)$. In this paper, we analyse the performance of the \emph{projected power method} (PPM) as a \emph{seeded} graph matching algorithm where we are given an initial partially correct matching (called the seed) as side information. We prove that if the seed is close enough to the ground-truth matching, then with high probability, PPM iteratively improves the seed and recovers the ground-truth matching (either partially or exactly) in $\mathcal{O}(\log n)$ iterations. Our results prove that PPM works even in regimes of constant $\sigma$, thus extending the analysis in (Mao et al. 2023) for the sparse Correlated Erdos-Renyi(CER) model to the (dense) CGW model. As a byproduct of our analysis, we see that the PPM framework generalizes some of the state-of-art algorithms for seeded graph matching. We support and complement our theoretical findings with numerical experiments on synthetic data.

==> Problem_statement.tex <==
\section{Problem statement}
The aim of \emph{graph matching} is to find, given two graphs $G=(V(G),E(G))$ and $H=(V(H),E(H))$ of equal size as input, a bijective function between $V(G)$ and $V(H)$ such that the alignment of the adjacency matrices is maximized. More formally, if $A$ and $B$ are the adjacency matrices of $G$ and $H$ respectively, we want to solve the following optimization problem:

\begin{equation}\label{form:1}
    \max_{x\in \mathcal{S}_n}\sum_{i,j}A_{ij}B_{x(i)x(j)}\tag{P1}
\end{equation}
where $\mathcal{S}_n$ is the set of all permutations of $[n]:=\{1,\cdots,n\}$. The objective function in \eqref{form:1} is called the \emph{adjacency agreement} for a given permutation $x\in\mathcal{S}_n$. Notice that if the graphs are $G$ and $H$ are isomorphic, then the maximal adjacency agreement has value $2|E|$ and is attained by any isomorphism $x\in\mathcal{S}_n$.  %Observe that  $0$ if and only if the graphs with adjacency matrices $A$ and $B$ are isomorphic. 

In matrix language, the problem \eqref{form:1} can be rewritten in the form
\begin{equation*}
    \max_{X\in \mathcal{P}_n}\langle A,X BX^T\rangle_F
\end{equation*}
where $\mathcal{P}_n$ is the set of permutation matrices of size $n$ and $\langle \cdot,\cdot\rangle_F$ is the Frobenius inner product in the space of $n\times n$ matrices. Observe that \eqref{form:1} is a well defined problem not only for adjacency matrices, but for any pair of matrices of the same size. Moreover, this is an instance of the well-known \emph{quadratic assignment problem}, which is combinatorially hard problem (known to be NP-hard in the worst case). 

It will be often useful to consider the ``lifted'' (or vector) formulation of the problem, where we identify a matrix in $\mathbb{R}^{n\times n}$ with a vector in $\mathbb{R}^{n^2}$. For matrix $X\in \mathbb{R}^{n\times n}$ we denote $[X]$ the vector in $\mathbb{R}^{n^2}$, where the columns of $X$ has been stacked together. It is easy to see that \eqref{form:1} can be written in the vector form as follows 

\begin{equation}
    \label{form:1'}
    \max_{[X]\in [\mathcal{P}_n]}[X]^TB\otimes A[X]\tag{P1'}
\end{equation}
where $[\mathcal{P}_n]$ is the set of permutation matrices in vector form.


Even if graph matching is known to be intractable in the worst case and the related \emph{graph isomporphism} problem has unkown complexity, both can be solved efficiently for many particular instances. Indeed, in \citep{RG_Isom_BES} the authors provide an algorithm that check if two graph are isomorphic in linear (on the number of edges) time and succeed for ``almost all graphs''. The latter can be rephrased as ``the algorithm works with high probability if the graphs are chosen uniformly'', which is equivalent to restrict ourselves to graphs generated by means of the Erdos-Renyi model $G(n,\frac12)$, where each edge appears with probability $1/2$ and all edges are decided independently. Our goal is of similar nature, that is to propose an efficient algorithm for the graph matching problem and study its statistical guarantees for a class of random graphs models.




==> models.tex <==
\section{Models for correlated random graphs}\label{sec:RGmodels}

Most of theoretical statistical analysis for the graph problem has been done so far for two random graph models: the \emph{correlated Erdos-Renyi} and the \emph{correlated Wigner model}. In those models the dependence between the two graphs $A$ and $B$ is explicitly described by the inclusion of a ``noise'' parameter. The main differences between both models are that the graph generated by the correlated Wigner generate a complete weighted random graph, with Gaussian weights, and the correlated Erdos-Renyi generate graphs with $\{0,1\}$ weights. 

\textbf{Gaussian Wigner model $W(n,\sigma,x^*)$}: The problem of graph matching \eqref{form:1} is well defined for matrices that are not necessarily adjacencies, so a natural extension is to consider two complete weighted graphs to be matched. In this direction, one model that has been proposed ,and analysed, is the Gaussian Wigner model, see \citep{Grampa} for example. Here we assume that $A$ and $B$ are symmetric matrices with i.i.d Gaussian entries (except for the symmetry constraint) and there is a linear relation between them. More specifically, we assume that \[A_{ij}\sim\begin{cases}\calN(0,\frac1n)\text{ if }i\neq j\\ \calN(0,\frac2n)\text{ if }i= j\end{cases}.\]
and $B_{x^*(i)x^*(j)}=\sqrt{1-\sigma^2}A_{ij}+\sigma Z_{ij}$, where the $Z_{ij}$ are the entries of a multivariate standard Gaussian matrix. Both $A$ and $B$ are distributed as the GOE (Gaussian orthogonal ensemble). Here the parameter $\sigma>0$ should be interpreted as the noise parameter ($B$ is a ``noisy perturbation'' of $A$).


\textbf{Correlated Erdos-Renyi $G(n,q,s,x^*)$:} for $q,s\in[0,1]$, the correlated Erdos-Renyi, with latent permutation $x^*\in \calS_n$, can be described in two steps: 
\begin{enumerate}
    \item $A$ is generated according to the Erdös-Renyi model $G(n,q)$.
    \item Conditional to $A$, the entries of $B$ are i.i.d according to the law: \begin{equation}
        B_{x^*(i),x^*(j)}\sim\begin{cases}
        Bern(s)\quad \text{if}\quad A_{ij}=1,\\
        Bern\big(\frac{q}{1-q}(1-s)\big)\quad \text{if } A_{ij}=0
        \end{cases}.
    \end{equation}
\end{enumerate}
Another way to describe this model is the following: first sample a ``mother'' graph according to the Erdos-Renyi model with parameter $\frac qs$ and then generate $A_{ij}$ and $B_{x^*(i)x^*(j)}$ independently by choosing to keep or not the corresponding edge in the mother graph with probability $s$ (if $s=0$ we consider that $A$ and $B$ are independent $G(n,q)$ graphs). In this model, we can interpret the parameter $s$ as the amount of noise that exists between $A$ and $B$, considering one a perturbation of the other. Indeed, when $s=1$ we have that $A$ and $B$ are indeed isomorphic and for $s=0$, $A$ and $B$ are independent. 



%\textbf{Correlated Gaussian mixtures model $CGM(n,\sigma,\nu,x^*)$}: We consider the following of correlated weighted graphs. Consider $\nu=\frac12\delta_{\nu_1}+\frac12\delta_{\nu_2}$, where $\nu_1,\nu_2\in \mathbb{R}$ and $\{Y_{ij},Z_{ij}\}^n_{i,j=1}$ two sets of independent $\calN(0,1)$ variables (except for the symmetry constrains $Y_{ij}=Y_{ji}$, $Z_{ij}=Z_{ji}$). Let  \begin{align*}
 %   A_{ij}&=U_{ij}+Y_{ij}\\
 %   B_{x^*(i)x^*(j)}&=U_{ij}+(\sqrt{1-\sigma^2}Y_{ij}+\sigma Z_{ij})
%\end{align*}
%where $U_{ij}\sim \nu$. Notice that each entry of $A$ and $B$ comes from (correlated) Gaussian location mixtures distribution with two components.
\ea{21/03: we are leaving the CGMixtures for the next time, right?.}
%\todo{Add motivation the Gaussian mixtures model.}

